K-Space Transformer for Undersampled MRI Reconstruction

This paper considers the problem of undersampled MRI reconstruction. We propose a novel Transformer-based framework for directly processing signal in k-space, going beyond the limitation of regular grids as ConvNets do. We adopt an implicit representation of k-space spectrogram, treating spatial coordinates as inputs, and dynamically query the sparsely sampled points to reconstruct the spectrogram, i.e. learning the inductive bias in k-space. To strike a balance between computational cost and reconstruction quality, we build the decoder with hierarchical structure to generate low-resolution and high-resolution outputs respectively. To validate the effectiveness of our proposed method, we have conducted extensive experiments on two public datasets, and demonstrate superior or comparable performance to state-of-the-art approaches.

==> ablation-tab.tex <==
\begin{table}
\setlength\tabcolsep{8pt}  
\centering
\resizebox{.87\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc}
\hline
\multicolumn{2}{c|}{Modules} & \multicolumn{2}{c|}{Gaussian 2D 5$\times$} &  \multicolumn{2}{c|}{Uniform 1D 5$\times$} & \multicolumn{2}{c}{Uniform 1D 2.5$\times$} \\ \hline
\ \ \ LRD \ \ \ & \ \ \ RM \ \ \ & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
\Checkmark & \Checkmark & 37.47 & 0.9823 & 31.50 & 0.9528 & 36.32 & 0.9848\\ 
\Checkmark & \XSolidBrush & 32.97 & 0.9337 & 27.52 & 0.8876 & xx.xx & 0.xxxx\\ 
\XSolidBrush & \XSolidBrush & 28.53 & 0.8416  & 21.31 & 0.6114 & xx.xx & 0.xxxx\\ \hline
\end{tabular}
}
\vspace{5pt}
\caption{Quantitive ablation study on critical designs.}
%\vspace{-1cm}
\label{tab:2}
\vspace{-5pt}
\end{table}

==> baseline-tab-align.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\vspace{-15pt}
\begin{table}[!htb]
\centering
\setlength\tabcolsep{5pt}  
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccc|cccc}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{Method}} & \multicolumn{6}{c|}{OASIS} & \multicolumn{4}{c}{fastMRI} \\ \cline{2-11} 

\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{10 $\times$} & \multicolumn{2}{c|}{5 $\times$} & \multicolumn{2}{c|}{2.5 $\times$} & \multicolumn{2}{c|}{5 $\times$} & \multicolumn{2}{c}{2.5 $\times$} \\ \cline{2-11} 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c}{SSIM} \\ \hline

K-UNet & \multicolumn{1}{c|}{xx.xx}  & \multicolumn{1}{c|}{0.xxxx} & \multicolumn{1}{c|}{24.53} & \multicolumn{1}{c|}{0.7808} & \multicolumn{1}{c|}{26.50} & 0.8483 & \multicolumn{1}{c|}{24.68} & \multicolumn{1}{c|}{0.6058} & \multicolumn{1}{c|}{26.99} & 0.7223 \\ \hline

Deep ADMM & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{0.xxxx} & \multicolumn{1}{c|}{26.03} & \multicolumn{1}{c|}{0.7202} & \multicolumn{1}{c|}{29.95} & \multicolumn{1}{c|}{0.8165} & \multicolumn{1}{c|}{24.43} & \multicolumn{1}{c|}{0.6172} & \multicolumn{1}{c|}{29.84} & \multicolumn{1}{c}{0.7838} \\ \hline

SwinMR & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{0.xxxx} & \multicolumn{1}{c|}{27.17} & \multicolumn{1}{c|}{0.9041} & \multicolumn{1}{c|}{29.83} & \multicolumn{1}{c|}{0.9435} & \multicolumn{1}{c|}{26.01} & \multicolumn{1}{c|}{0.6684} & \multicolumn{1}{c|}{29.10} & \multicolumn{1}{c}{0.7842} \\ \hline

UNet & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{0.xxxx} & \multicolumn{1}{c|}{27.53} & \multicolumn{1}{c|}{0.8895} & \multicolumn{1}{c|}{29.05} & 0.8988 & \multicolumn{1}{c|}{26.72} & \multicolumn{1}{c|}{0.6835} & \multicolumn{1}{c|}{29.81} & 0.7983 \\ \hline

D5C5 & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{0.xxxx} & \multicolumn{1}{c|}{27.66} & \multicolumn{1}{c|}{0.8895} & \multicolumn{1}{c|}{32.48} & 0.9615 & \multicolumn{1}{c|}{26.87} & \multicolumn{1}{c|}{0.6793} & \multicolumn{1}{c|}{30.64} & 0.8126 \\ \hline

OUCR & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{0.xxxx} & \multicolumn{1}{c|}{29.52} & \multicolumn{1}{c|}{0.9310} & \multicolumn{1}{c|}{33.75} & 0.9709 & \multicolumn{1}{c|}{27.71} & \multicolumn{1}{c|}{0.7009} & \multicolumn{1}{c|}{30.95} & 0.8168 \\ \hline

Ours & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{0.xxxx} & \multicolumn{1}{c|}{\textbf{31.50}} & \multicolumn{1}{c|}{\textbf{0.9528}} & \multicolumn{1}{c|}{\textbf{36.32}} & \textbf{0.9848} & \multicolumn{1}{c|}{\textbf{27.80}} & \multicolumn{1}{c|}{\textbf{0.7078}} & \multicolumn{1}{c|}{\textbf{31.04}} & \textbf{0.8189} \\ \hline
\end{tabular}}
\vspace{-5pt}
\caption{Quantitative comparison on uniform 1D sampling pattern~(align if possible)}
\label{tab:uniform}
\vspace{-12pt}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\centering
\setlength\tabcolsep{5pt}  
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccc|cccc}
\hline
\multirow{3}{*}{Method} & \multicolumn{6}{c|}{OASIS} & \multicolumn{4}{c}{fastMRI} \\ \cline{2-11} 
 & \multicolumn{2}{c|}{10 $\times$} & \multicolumn{2}{c|}{5 $\times$} & \multicolumn{2}{c|}{2.5 $\times$} & \multicolumn{2}{c|}{5 $\times$} & \multicolumn{2}{c}{2.5 $\times$} \\ \cline{2-11} 
 & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & SSIM & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & SSIM \\ \hline
%Input & \multicolumn{1}{c|}{20.99} & \multicolumn{1}{c|}{0.4856} & \multicolumn{1}{c|}{23.99} & \multicolumn{1}{c|}{0.5941} & \multicolumn{1}{c|}{26.92} & \multicolumn{1}{c|}{0.6936} & \multicolumn{1}{c|}{25.01} & \multicolumn{1}{c|}{0.5951} & \multicolumn{1}{c|}{27.54} & 0.7254 \\ \hline
K-UNet & \multicolumn{1}{c|}{25.34} & \multicolumn{1}{c|}{0.766} & \multicolumn{1}{c|}{28.76} & \multicolumn{1}{c|}{0.8427} & \multicolumn{1}{c|}{33.96} & 0.9288 & \multicolumn{1}{c|}{27.15} & \multicolumn{1}{c|}{0.6696} & \multicolumn{1}{c|}{28.90} & 0.7710 \\ \hline

Deep ADMM & \multicolumn{1}{c|}{26.17} & \multicolumn{1}{c|}{0.7312} & \multicolumn{1}{c|}{30.41} & \multicolumn{1}{c|}{0.8122} & \multicolumn{1}{c|}{33.94} &\multicolumn{1}{c|}{0.8513}  & \multicolumn{1}{c|}{29.31} & \multicolumn{1}{c|}{0.7515} & \multicolumn{1}{c|}{30.97} &  \multicolumn{1}{c}{0.8162}\\ \hline

SwinMR & \multicolumn{1}{c|}{27.48} & \multicolumn{1}{c|}{0.8893} & \multicolumn{1}{c|}{30.36} & \multicolumn{1}{c|}{0.9341} & \multicolumn{1}{c|}{33.75} &\multicolumn{1}{c|}{0.9659}  & \multicolumn{1}{c|}{28.41} & \multicolumn{1}{c|}{0.7080} & \multicolumn{1}{c|}{30.30} &  \multicolumn{1}{c}{0.7949}\\ \hline

UNet & \multicolumn{1}{c|}{27.63} & \multicolumn{1}{c|}{0.8437} & \multicolumn{1}{c|}{31.27} & \multicolumn{1}{c|}{0.9024} & \multicolumn{1}{c|}{35.02} & 0.9388 & \multicolumn{1}{c|}{28.33} & \multicolumn{1}{c|}{0.7120} & \multicolumn{1}{c|}{31.35} & 0.8283 \\ \hline

D5C5 & \multicolumn{1}{c|}{30.51} & \multicolumn{1}{c|}{0.9241} & \multicolumn{1}{c|}{35.91} & \multicolumn{1}{c|}{0.9743} & \multicolumn{1}{c|}{42.72} & 0.9927 & \multicolumn{1}{c|}{29.78} & \multicolumn{1}{c|}{0.7507} & \multicolumn{1}{c|}{32.00} & \textbf{0.8399} \\ \hline
OUCR & \multicolumn{1}{c|}{31.61} & \multicolumn{1}{c|}{0.9442} & \multicolumn{1}{c|}{36.78} & \multicolumn{1}{c|}{0.9797} & \multicolumn{1}{c|}{42.80} & 0.9933 & \multicolumn{1}{c|}{\textbf{29.95}} & \multicolumn{1}{c|}{0.7522} & \multicolumn{1}{c|}{\textbf{32.04}} & 0.8382 \\ \hline
Ours & \multicolumn{1}{c|}{\textbf{32.58}} & \multicolumn{1}{c|}{\textbf{0.9529}} & \multicolumn{1}{c|}{\textbf{37.47}} & \multicolumn{1}{c|}{\textbf{0.9823}} & \multicolumn{1}{c|}{\textbf{43.68}} & \textbf{0.9946} & \multicolumn{1}{c|}{29.88} & \multicolumn{1}{c|}{\textbf{0.7534}} & \multicolumn{1}{c|}{31.97} & 0.8389 \\ \hline
\end{tabular}%
}
\vspace{-5pt}
\caption{Quantitative comparison on Gaussian 2D sampling pattern}
\label{tab:gaussian}
\vspace{-15pt}
\end{table}
